Understanding the Practice, Perception, and Challenge of Blind or Low Vision Students Learning through Accessible Technologies in Non-Inclusive 'Blind Colleges'

In developing and underdeveloped regions, many 'Blind Colleges' exclusively enroll individuals with Blindness or Vision Impairment (BLV) for higher education. While advancements in accessible technologies have facilitated BLV student integration into 'Integrated Colleges,' their implementation in 'Blind Colleges' remains uneven due to complex economic, social, and policy challenges. This study investigates the practices, perceptions, and challenges of BLV students using accessible technologies in a Chinese 'Blind College' through a two-part empirical approach. Our findings demonstrate that tactile and digital technologies enhance access to education but face significant integration barriers. We emphasize the critical role of early education in addressing capability gaps, BLV students' aspirations for more inclusive educational environments, and the systemic obstacles within existing frameworks. We advocate for leveraging accessible technologies to transition 'Blind Colleges' into 'Integrated Colleges,' offering actionable insights for policymakers, designers, and educators. Finally, we outline future research directions on accessible technology innovation and its implications for BLV education in resource-constrained settings.

==> Workshop_Study.tex <==
\section{Workshop Study}
\subsection{Methods}
In this paper, we conducted a workshop study involving 9 BLV students, approved by the Institutional Review Board (IRB), aimed at understanding their computer usage in real learning scenarios and identifying potential computer accommodations that could be added to support their learning. 
\input{Table/Table1}
\subsubsection{Participants}
The participants in this study were recruited from a Chinese public university with a collaborative relationship with our research lab. The students were specifically admitted through the special education department. The detailed information regarding the student's age (M = 24.1; SD = 1.70), gender (4 Male; 5 Female), degree of visual impairment (8 totally blind; 1 low vision), field of study (8 Acupuncture and Tuina Science (ATS); 1 Music) and educational level (5 Undergraduate; 4 Graduate), is provided in table 1. Each participant signed a consent form for their involvement in this study and received compensation of 300CNY for their time.

\subsubsection{Procedure}
We conducted this study within the familiar classroom setting of the participants’ university. The study consists of five different sections, separated by two 5-minute breaks (see Figure 2). We first distributed the syllabus and PowerPoint materials, introducing the workshop’s agenda and the context of the lesson. Participants were also given instructions on downloading virtual meeting software. Following, participants connected to a virtual meeting room, where we invited an HCI Professor to deliver a 30-minute online lecture on the interdisciplinary design for accessibility and HCI. In the third session, students were grouped into three and assigned tasks to collaborate and create a presentation demonstrating their learning preference in summarization, research, and collaboration (refer to Appendix 1 for detailed task instruction). Each group would deliver their finding, with presentations lasting approximately 10-20 minutes each. Finally, we conducted focus group interviews for each group, asking students with opening questions in three aspects, their experience of the workshop, their operation preferences on computers and strategies they use when facing challenges. The process of the workshop could be visualized in Figure \ref{fig:Flowchart}, including each of the five steps and the approximate time for each section. Each section is color-coded with different colors.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figure/Flowchart.png}
    \caption{\textbf{This flowchart illustrate the procedure of workshop study with the approximated time. }}
    \Description{The picture shows the flowchart for this Workshop procedure arrangement. The flowchart consists of a rectangle and some markup. The rectangle shows the duration of each session of the workshop, and the name of each session is labeled below the duration. From left to right they are: Preparation and Preview Coursework (15 minutes), Online Class (20 minutes), Break (5 minutes), Discussion and Group Work (60 minutes), Presentation (40 minutes), Break (5 minutes) and Focus Group Interview (45 minutes).}
    \label{fig:Flowchart}
\end{figure}

\subsubsection{Data Collection and Analysis}
Throughout the workshop, with the participants’ consent, we captured their screen activities, observed and recorded their computer operation, and audio-recorded the focus group discussions. We particularly emphasized identifying actions by participants that were either intriguing or relative to our research. These actions served as focal points for our focus group interviews, where participants provided insights into the reasons behind their observed behaviors, adding depth and insights. For data analysis, we followed ground theory \cite{corbin1990basics} with an open-coding and affinity diagramming approach, which was applied to both the focus group interview transcript and behavior analysis. Two researchers first open-coded all the videos, mainly coding the operations on a computer, and then matched relevant interview answers to uncover participants’ reasons for practice. They subsequently address conflicts of their conceptions, achieving consensus on their codes. The codes would then conduct an affinity diagram on the consolidated codes, generating patterns that would be categorized into themes. Finally, we generated some key themes following four sessions. The description and analysis of the theme will be addressed in the following section. 


\subsection{Findings: The practice of BLV students using computers in the course context}
In this section, we will report a comprehensive account of what specific situations and how BLV students would choose to use computers during various workshop sessions. It is worth noting that this section will more likely emphasize the selection of applications or software, outlining their intended purposes, and we only explain operations and strategies employed by the students through the combination of observation and interview analysis. For a broad overview of blind students' general computer usage, which will not be reported to avoid redundancy, please consult Section 2.2.

\subsubsection{Session1: Preparation and Preview Coursework}
In general, we found that preview is crucial for BLV Students, they usually set up their computers and preview their class materials by screen reader software or OCR 
 software before class to help them gain a better understanding of their knowledge in the classroom. Two essential things take their priority to check for them: the first is improving the efficiency of lessons by using external devices and adjusting computer settings, and the second is addressing accessibility design shortcomings during unfamiliar software login. %%(外接）设备使用和无障碍系统登入(其实这里可以讲一下他们遇到的困难，感觉现在这里全是正面的内容）

We found that BLV students would like to bring an external keyboard rather than a laptop keyboard for class (Fig.\ref{fig:figure3}-1). They indicated that external keyboards help them quickly type down notes and the keypad is a tricky way to overcome accessibility issues with some software (S1, S5, S6, S8). 
 
\begin{quote}
    \textit{S8: ``...The external keyboard has bigger keys and I'll be able to type faster. The external keyboard will also have a keypad, which I can use to simulate the layout selection of a mouse to select focus more easily and make operations more efficient...''}
\end{quote}

    Besides,they will use OCR software when BLV students encounter unreadable content (Fig.\ref{fig:figure3}-8).

\begin{quote}
    \textit{S2: ``...We will use OCR to recognize all the text on the screen, and then use the arrow keys to navigate between the text to find what we’re looking for. For example, if I want to find the mute button, I identify the word ’mute’ through OCR and then use specific keyboard keys to perform a click action, ultimately achieving my objective...''}
\end{quote}

They also adjust the volume and speed of the screen reader before class to ensure that screen-reading does not interfere with listening to the teacher's lectures in class (S1, S8). Before the class, a series of software of the same type was tested for accessibility to select the best software to use on the computer (S5, S7). BLV students ingeniously deploy Optical Character Recognition (OCR) technology to transform PDF files and images into text formats and send translated documents to their classmates in order to minimize challenges associated with both previewing and retrieving information (S4, S7). Furthermore, these students take advantage of previews to identify key focal points, enabling them to swiftly take notes without disrupting their auditory impairments are not able to accurately determine the switch of the camera and microphone through the screen-reading function, however, they are worried that the function will be turned on by mistake, which makes blind students very careful when they use the software (S1, S7).

BLV students were also required to open some software in advance to prepare for class. The main problems they had with using software were the graphic validation (Fig.\ref{fig:figure3}-4) and advertisement pop-ups (S1~S9).

\begin{quote}
    \textit{S1: ``...When it comes to graphical validation for logging in, we can't accomplish this task because we don't have a way to perceive the graphic through screen-reading software, not to mention manipulating the graphic to complete the authentication...''}
\end{quote}

When BLV students have successfully logged into the software, they may also encounter pop-up advertisements that will appear on the software (Fig.\ref{fig:figure3}-5). These pop-up advertisements may affect the smooth use of the software by BLV students, and sometimes BLV students may accidentally click on the pop-up advertisements and be redirected to the advertised web pages (Fig.\ref{fig:figure3}-6), which may affect the efficiency of BLV students' use of the software.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figure/p11.png}
    \caption{\textbf{BLV students prepared computers and conducted preview, such as: (1) Connecting an external keyboard to a laptop, (2) Connecting headphones to the computer and put headphones on so BLV students can hear the sound of the screen reader, (3) Login to online meeting software by cell phone number, (4) Slider validation login, BLV students usually need help from others, (5) Encountering pop-up advertisements within the software after logging in to the software, (6) BLV students accidentally clicked on pop-up advertisements, jumped to advertised page, (7) Reading courseware with OCR recognition, and (8) OCR-recognized courseware contained text ordering confusion and was difficult to read.}}
    \Description{Eight images in a two-by-four format labelled (1), (2), (3), (4), (5), (6), (7) and (8) show BLV students prepared computers and conducted preview. Image (1) shows how a BLV student connected the external keyboard to a laptop. In (2) a male BLV student was wearing headphones with his left hand. In (3) the login window for the online conferencing software appeared in the middle of the computer screen, and a BLV student was logging into the software via a cell phone number. In (4) the slider validation window appeared in the middle of the computer screen, and the top half of the pop-up validation window was a graphic with missing pieces, and the bottom half was a slider bar that BLV students needed to drag to fill in the missing pieces. In (5) after passing the slider validation, the software appeared a pop-up advertisement advertising the software's recharge business. In (6) a BLV student accidentally clicked on a pop-up advertisement and the computer interface jumped to a web page that advertised the content of the advertisement. In (7) a BLV student used the computer, recognized the content of the lesson using OCR and pasted the content into Microsoft Word, which was on the left side of the computer interface, with the online conferencing software in the upper right corner, and a pop-up message from the system in the lower right corner. In (8) the computer interface showed the content of the courseware after it had been recognized by OCR, and there was a problem with the order of the text, which made it impossible to read it smoothly and correctly.}
    \label{fig:figure3}
\end{figure}
\subsubsection{Session2: Online Class}

For virtual courses to begin, most BLV students choose to reduce the distractions associated with operating the computer and focus entirely on the class.  Noticeably, most BLV students do not record notes but listen to the teacher's content (Figure \ref{fig:figure4}-1). Some BLV students mentioned that when using the computer, they have to listen to the class, the sound of the headset's screen reading, and think about the knowledge points at the same time. In that case, BLV students will have a conflict of information reception, which reduces the efficiency of listening to the class (S1). However, BLV students also claimed that they use computers to take few notes more in compulsory courses to help them review what they learned. In this situation, they prefer recording keywords rather than large content sections (Figure \ref{fig:figure4}-4), which they must memorize for their final exam (S1). One of the BLV students also explained his preferences for writing down keywords based on his judgment based on their previews and learning experiences (S8).
\begin{quote}
    \textit{S8: ``...I record keywords by my years of study experience, for example, if I feel that this content is a test point or a learning difficulty, I will simply write it down...''}
\end{quote}
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figure/p22.png}
    \caption{\textbf{BLV student behavior in class. (1) Five BLV students sitting in a row, using computers are listening to a lecture. (2) A BLV student operated computers through shortcuts. (3-1) A student with low vision used the magnifying glass function of the computer to read the courseware during class. (3-2) Blind students accessed information by quickly switching screens. (4) BLV students used the keyboard typing to record few keywords.} }
    \Description{The first four of the five images are laid out 2 by 2, with the fifth image on the last line. Five images are labelled (1), (2), (3-1), (3-2) and (4). In (1) five BLV students sat in a row and used computers and headphones for listening the class. In (2) a male BLV student is using an external keyboard and using shortcuts to switch software to access content from different software. In (3-1) a female low vision student was using the magnifying feature on her computer to read a lesson on her computer. In (3-2) the interface of the blind student's computer included two desktops, one for listening to the teacher's lessons and one for reading the lessons. In (4) a female BLV student was using a memo to record notes from class, which were very brief.}
    \label{fig:figure4}
\end{figure}


They also have different preferences in choosing note-taking software: BLV students take notes in plain text and most of them will choose Memo for Windows in order to open software and take notes more quickly (S1), while some will choose to use Microsoft Word because the recorded notes can be read on Microsoft Word on the cell phone so that they can get a better screen-reading experience on the cell phone. They also reported that they will reorganize their notes after the class by adding more information from files provided by teachers (S4, S7). 

\begin{quote}
    \textit{S1: ``...I would find what I wanted from the documents given by the teacher by using keywords recorded in class and organizing them more logically together...''}
\end{quote}

In addition, to further improve the efficiency of listening to teachers, BLV students have their strategies to improve the efficiency of computer using: creating multiple windows for different functional areas (Figure \ref{fig:figure4}-3-2) and switching between them (S2), using shortcut keys (Figure \ref{fig:figure4}-2) to quickly return to the desktop and using the search box to quickly search for software (S3, S8), using shortcuts to switch between programs to do different tasks (S7), and installing multiple plug-ins in the browser to improve efficiency (S8). 

\begin{quote}
    \textit{S7: ``...After using a screen reader on our computer, there will only be one focus on the computer, and if I don't do anything, the focus will only stay on one software. To access a lot of information at the same time, I would need to quickly switch interfaces so that the focus appears in different files...''}
\end{quote}

During online courses they also face many problems, mainly focusing on the accessibility design of the software, the limitations of the software technology, and the hardware properties of the computer itself. In the accessibility design, due to the commercialization of the software, there are a lot of pop-up advertisements and there is no focus for blind people to close pop-up advertisements (S7, S8). For the low-vision student, the magnification function (Figure \ref{fig:figure4}-3-1) is often difficult to use when online meetings going (S9). 
\begin{quote}
    \textit{S9: ``...When I use the zoom feature on my computer, it never zooms right into the area I want. There are times when it's hard to get subtle manipulation after zooming in because the mouse sensitivity is too fast with the screen zoomed in. As a result, I spend a lot of time every time when I want to read a part of the document...''}
\end{quote}

BLV students primarily rely on computer shortcuts but they will face some problems using shortcuts, for example: If BLV students change their computer system, the shortcuts will change and they cannot use shortcuts fluently. Besides, some software's shortcuts will interfere with the computer system's shortcuts which makes some shortcuts invalid (S9). BLV students are unable to understand three-dimensional images, and computers are unable to provide effective assistance (S1). 

\begin{quote}
    \textit{S7: ``...Our teachers usually use many metaphors to describe things that are unfamiliar to us to help us understand the size, shape, and structure of things. But in today's lesson, the teacher only said that the product was round, and the exact look of this product was still vague, not to mention its structure...''}
\end{quote}

%%For example, normal teachers usually use images to explain some complicated devices and describe the devices in few details. However, teachers specializing in classes for BLV students will use many metaphors to help student 

If BLV students are exposed to new concepts or unfamiliar things in the classroom, BLV students mentioned that they have low sensory ability and cannot fully understand the meaning (S4, S7). 

\subsubsection{Session3: Discussion and Groupwork}
In this session, students were given assignments to complete, and although we did not mandate the use of their devices. However, all students involuntarily use computers to complete all tasks indicating a preference for computer-based work.
%%在这里我们并不要求他们的设备使用，学生们根据自己要求进行选择使用电脑或手机。However，所有同学都不自主的使用电脑完成所有任务。
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figure/p33.png}
    \caption{\textbf{BLV students used computers to access information and complete tasks. (1) Nine students were divided equally into three groups and sat together for a discussion. (2) Two BLV students were discussing the division of labor. (3-1) A female BLV student was using the website to search for literature. (3-2) A male BLV student was using a computer to read a document and record notes at the same time. (3-3) A BLV student was trying to use ChatGPT to search for desired information. (3-4) Three BLV students were listening to a video together to understand the concepts. (4) Two BLV students were each organizing their content and trying to aggregate it together. (5) The BLV student in charge of creating the slides was reading others' materials and were ready to start creating the slides.}}
    \Description{Eight images in a two-by-four format labelled (1), (2), (3-1), (3-2), (3-3), (3-4), (4) and (5) show BLV students used computers to access information and complete tasks. In (1) the nine BLV students were divided equally into three groups and they sat together. Their groupings were labeled with boxes in the picture: Group 1, Group 2, and Group 3. In (2) a male BLV student was discussing team division of labor with a female BLV student. The male BLV student was saying, ``Let me do the report. I'll summarize what we found.'' The female BLV student replied, ``No problem. I'll put together an outline for you.''. In (3-1) a female BLV student wearing headphones was using a computer to find the paper she wanted on a paper search site. In (3-2) a male BLV student was using a computer to simultaneously read literature and record notes; the upper left corner of the computer screen was his memo used to record notes, and the rest of the screen was the area where he read literature. In (3-3) a male BLV student used the web page to open the OpenAI web page to try to use ChatGPT to assist him in searching for information.In (3-4) three BLV students were sitting on a row, the student on the far right had a cell phone that was playing a video, and all three students were listening to the sound of the video on their phones to learn something unfamiliar. In (4) a male BLV student and a female BLV student were summarizing the content they searched.The male BLV student was saying, ``The concept of my document is about concept.'' The female BLV student replied, ``My part is about design.''. In (5) a female low vision student was using her cell phone to read information sent by other students and using her computer to summarize the information and prepare a slide show.}
    \label{fig:figure.5}
\end{figure}

During the group work session, the method of assigning tasks to BLV students was similar to that of sighted university students (Figure \ref{fig:figure.5}-2). If a student was familiar with the specific software involved in the task, that student would take up this task (S1). Additionally, each student was responsible for producing a part information about their assigned task, which the group leader would then consolidate into a comprehensive outline (S4). The choice of group leader is voluntary for most time. However, unlike sighted individuals, they don't access co-working software to collaboratively complete tasks due to the absence of accessibility features in such software.

\begin{quote}
    \textit{S4:``...I really wish to experience real-time online collaborative office software like sighted individuals, to enhance efficiency and even engage in online learning with them...''}
\end{quote} 

When each student was working on the task, their biggest challenge was to search for information due to BLV people being unable to locate their targeted information and they can only filter them by listening to the text materials linearly (S1, S2, S5, S6, S7). Therefore, the time used by BLV students to find the desired content is often far greater than that of sighted people in information searching. When searching for simple answer content, most students chose to use Baidu, although they thought that Baidu \footnote{https://www.baidu.com/} provided a lot of advertisements and ineffective content. They chose to continue to use Baidu because they have used Baidu since they were children and are used to using this software (S6, S7, S9). While riding the wave of AI, some also attempted to use ChatGPT to search for information (S4, S5, S7)(Figure \ref{fig:figure.5}-3-3). However, they found that ChatGPT generated an amount of condescending and irrelevant content that led them to conduct a secondary search within ChatGPT, often wasting more time.

As for some professional and academic answers, all students use China Academic Journals \footnote{https://www.cnki.net/} to read papers(Figure \ref{fig:figure.5}-3-1), but BLV students can't use the advanced search function, which makes it impossible for them to find some papers quickly, as (S1). 

\begin{quote}
    \textit{S9: ``...Some difficult knowledge I will choose to listen to the video to understand, such as music knowledge in today's class, through the video I can listen to actual examples of music to better understand. And I like those videos that start straight to the point, which can save my time...''}
\end{quote}


%%这段内容我变成了quote：and hope that the most important information of the videos could be demonstrated at the beginning to improve the efficiency of learning new concepts (S8, S9)
Navigating image-based contexts, they often found that it took longer than expected because the only way of accessing information was through OCR recognition to read the text (S1, S6, S7); However, this approach could not fix all the imaged-based problems. For example, some foreign language websites, after translating the websites into Chinese, some images  still contain a mix of Chinese and English, also resulting in recognized difficulties for OCR (S6); Although they acknowledge there are many plug-in accessibility technologies to assist in accessing the information, they often do not know how to install them and believed there is a high learning cost greater than the speed of plugin updates and replacements (S4).

After getting the desired information, the next for BLV students is to organize their separately collected information information. They may organize information from both taught on the course and searched from the internet. Some BLV students presented that they may use AI technology such as ChatGPT to quickly find the core content and exclude repeated content from a large number of text materials, thus reducing the time of reading (S4, S7). 

However, they have many needs when organizing information. One of the primary needs is to establish a shared understanding with their peers. They are usually confused about whether their ideas align with others in the aspect of presentation framework. Thus, they desire to utilize mind map software to create a structure for homework and presentation (S4). However, existing mind map software presents challenges for BLV students due to they could not receive the visual input of sections and subsections, making it difficult for them to comprehend (S4). 

\begin{quote}
    \textit{S4: ``...When I use current mind mapping software, if I use screen readers, I just read pieces of information. I cannot know the relationships of each knowledge point, such as juxtaposition and inclusion. In addition, nowadays mind maps are more of a pictorial presentation, so it leads to my inability to create such diagrams as I can't see...''}
\end{quote}

\subsubsection{Session4: Presentation}
%修齐，这里的任务开头需要你写一下，你比较专业lol
In the final presentation session, each group choose to use PowerPoint to do the presentation (Figure \ref{fig:figure.6}). Some BLV students expressed reservations about PowerPoint, perceiving it was made only to be presented to others sighted, therefore exhibiting resistance to making PowerPoint for most of the class (S7).  However, all the BLV students share a common concern that their PowerPoint doesn't appear visually appealing due to they could not add photos and animations which they believed would affect the quality of the presentation (S1-S9). 
\begin{quote}
    \textit{S7: ``...PowerPoint is only made for people with eyesight, we can't get benefits from it. Besides, it is inconvenient to do PowerPoint, forcing us to do PowerPoint makes me feel that the teacher is making it difficult for us...''}
\end{quote}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figure/p44.png}
    \caption{Three BLV students were together for a group report. The student sitting on the far right was debriefing and the student sitting in the center controlled the slides.}
    \Description{Three BLV students were together for a group report. The student sitting on the far right was debriefing and the student sitting in the center controlled the slides.}
    \label{fig:figure.6}
\end{figure}
Such negative feelings came from the inconvenience of making PowerPoint. For example: BLV students could not perceive the positional relationship between multiple text boxes on a page of PowerPoint, which could easily lead to the superimposition of textual content (S1, S4, S6). Meanwhile, they have no idea about where to put the pictures when placing them (S1). To solve these problems, BLV students usually resort a templates to edit all PowerPoint (S4) or seek peers or pay someone to help them beautify the document (S1, S4). In this workshop, All three groups chose to utilize a simple white template with textual content, without any charts and animations.

BLV students mentioned that they typically use two computers, one for sharing the screen and the other to read the contents of PowerPoint to help them memory speech outlines (S1, S7, S8). Therefore, during this process, BLV students usually wear a headphone to listen to the screen reading information (S4), or they may seek assistance from other people to operate the computer to navigate the PowerPoint for them (S4). However, they also expressed concerns about the delay in page-turning, primarily because BLV students were unsure if the person assisting them was synchronizing the page changes with their speech (S2, S3). In this workshop, one student from each group came out to give the presentation and smoothly operated the PowerPoint on their own to turn the pages.

However, they also encountered some problems with daily presentations. For example, they may face some unexpected animations in their PowerPoint, which often leads to a misalignment of the presentation as the presentation does not correspond to the PowerPoint (S5, S6); Additionally,  when using sighted people's computers in the classroom to deliver their presentations, those computers did not support screen-reading functions, which would affect the delivery of the presentations (S6). Moreover, BLV students cannot know the attitudes and emotions of the quiet audience on stage when they give a speech, and thus cannot adjust the pace of the presentation (S4). In order to avoid those above problems, BLV students documents of presentations typically prepare plain text documents for their presentations like they made in our workshop (S7, S8), while some students also add music or sound effects into PowerPoint to remind themselves which page they are presenting and trying to give audiences a better experience (S6).
